Computational Approaches for Exponential-Family Factor Analysis

We study a general factor analysis framework where the $n$-by-$p$ data matrix is assumed to follow a general exponential family distribution entry-wise. While this model framework has been proposed before, we here further relax its distributional assumption by using a quasi-likelihood setup. By parameterizing the mean-variance relationship on data entries, we additionally introduce a dispersion parameter and entry-wise weights to model large variations and missing values. The resulting model is thus not only robust to distribution misspecification but also more flexible and able to capture mean-dependent covariance structures of the data matrix. Our main focus is on efficient computational approaches to perform the factor analysis. Previous modeling frameworks rely on simulated maximum likelihood (SML) to find the factorization solution, but this method was shown to lead to asymptotic bias when the simulated sample size grows slower than the square root of the sample size $n$, eliminating its practical application for data matrices with large $n$. Borrowing from expectation-maximization (EM) and stochastic gradient descent (SGD), we investigate three estimation procedures based on iterative factorization updates. Our proposed solution does not show asymptotic biases, and scales even better for large matrix factorizations with error $O(1/p)$. To support our findings, we conduct simulation experiments and discuss its application in four case studies.

==> orient-stats.tex <==
% maybe helpful to talk about constraint on manifold, riemannian manifold to Stiefel manifold
\section{Orientation Statistics and Factor Identifiability}
\label{sec:ori_stat}
\subsection{Orientation Statistics}
\label{subsec:ori_stat_intro}
 Modeling data from an orientational perspective has a long history in statistics with the motivation that data of various fields have been shown to be directional in nature. For example, in natural language processing, cosine similarity on the words embedding is essentially a scaled inner product, which has been modeled by von Mises-Fisher distribution in \citep{2005text_direct} and \citep{2007text_direct}. In gene studies, \citep{2003gene_dir} shows that anti-correlated gene expression pattern could indicate functional similarity and recent paper \citep{2021gene_dir} proposed clustering algorithm based upon von Mises-Fisher setup. For circular data that can be effective measured with angles\citep{2009direct_textbook}, the orientation of a loop on cardiograph was studied in \citep{1972orient_stat} and \citep{1977mises}. The microphone array was studied to facilitate multiple-target tracking in \citep{2014voice_track}. Recent researches have been generalizing the orientational statistics to bayeisan setup \citep{2009dir_mc} and supplied with efficient MCMC algorithm \citep{2021dir_mc}.

Mathematically, orientational statistics assumes that $n$ rows of $p$ dimensional matrix $(X)_{n\times p}$ effectively lies on a rigid configuration of distinguishable directions\citep{1972orient_stat}, which can be characterized via an inner product with a positive definite matrix $C\in \mathbb{R}^{p\times p}$ to provide angle(direction) specification $(X^\top X =C)$. From a differential geometry perspective, the orientational statistics constraints the $n\times p$ Riemann space by $X^\top X = C$ and form the Stiefel-C manifold $S(C)$. The Stiefel-C manifold $S(C)$ is then characterized by a rank $q(q\leq p)$ $n\times p$ matrix $(F)_{n\times p}$, which entitles the following formal definition of von Mises-Fisher \textbf{Matrix} distribution:
\begin{definition}
For $n\times p$ random matrix X satisfying $X^\top X = C$, X is said to be distributed as von Mises Fisher Matrix distribution $D(C,F)$ given parameter $p\times p$ matrix $C$, normalization constant $a(c,F)$ and $n\times p$ matrix $F$, if the density of data X follows:
\begin{equation}
    \label{eq:direct_mstat}
    \begin{aligned}
        D(C,F) &= a(C,F) \exp(tr(F^\top X), X\in S(C)\\
        &\propto \exp(tr(F^TX), X\in S(C)
    \end{aligned}
\end{equation}
\end{definition}
\begin{remark}
For $n=1, C= I_p$, Stiefel-C manifold $S(I_p)$ is abbreviated as Stiefel manifold and Eq \ref{eq:direct_mstat} is reduced to the von Mises-Fisher distribution with $\kappa>0, a_{\kappa}(I_p,F) = \frac{\kappa^{d/2-1}}{(2\pi)^{p/2} I_{p/2-1}(\kappa)}$: 
\begin{equation}
    \label{eq:direct_stat}
    \begin{aligned}
        f(X_i) = a_{\kappa}(I_p, F)\exp(\kappa F^\top X_i)
    \end{aligned}
\end{equation}
\end{remark}



\begin{definition}
For $n\times p$ deterministic matrix F, the $n\times p$ matrix M and $ p\times p$ matrix K are called polar C form of F with M the polar component(mean direction) and K the elliptic component(concentration) if $M$ and $K$ satisfies:
\begin{enumerate}
    \item $F =MK$
    \item $M^\top M = C$
    \item $K$ is symmetric positive definite
\end{enumerate}
\end{definition}
\begin{remark}
The polar component $M$ has the interpretation of mean direction and the elliptic component has the interpretation of concentration. This can be easily seen in the one dimensional Mises Fisher distribution in Eq~\eqref{eq:direct_stat} where $\kappa$ is the concentration and vector $F$ as the mean direction. \citep{1972orient_stat} gives more a detailed proof to connect Mises Fisher Matrix distribution to multivariate gaussian with parameter $M$ and $K$, which preserves such interpretations.
\end{remark}

\citep{1972orient_stat} also derived some important properties about the Von-Misers Fisher Matrix distribution. For the coherence of our discussion, we here only summarize some of the properties that are useful to construct our DMF setup and refer the readers to Down's origin paper for more detailed discussion and rigorous proof.
\begin{property}
\label{prop1}
The Von-Misers Fisher Matrix distribution parameter matrix $F$ entitles unique polar C form with the folllowing identification:
    \[
\begin{split}
F =  \underbrace{(F C^{\frac{1}{2}} (C^{\frac{1}{2}}F^T FC^{\frac{1}{2}})^{-\frac{1}{2}}C^{\frac{1}{2}})}_{M}
\underbrace{(C^{\frac{1}{2}}K C^{\frac{1}{2}})}_{K},
\end{split}
\]
where for semi-positive definite matrix C with eigen representation $C = \theta D^2\theta^\top$, $C^{1/2} = (\theta D^2\theta^\top)^{\frac{1}{2}} = \theta D \theta^\top$. The Von-Mises Fisher Matrix distribution could thus be equivalently written as $D(C,F) \equiv D(C,KM)$
\end{property}
%
\begin{property}
\label{prop2}
The von-Misers Fisher Matrix distribution is closed under left orthogonal and right invertible transformation. Specifically, if $X\sim D(C,F))$, then for $n\times n$ orthogonal matrix $L$ and $p\times p$ invertible matrix $R$, the transformed random matrix $LXR$ follows:
    $$LXR \sim D(R^\top C, (LMR)(R^{-1}K(R^{-1})^\top))$$
\end{property}
%
\begin{property}
\label{prop3}
For $n$ rows of independent multivariate dimension $p$ Gaussian with means equal to $n$ rows of $n\times p$ matrix $M$ and common dispersion parameter $K^{-1}$, The random matrix $X$ given the condition $X^\top X = C$ is distributed as Von-Mises-Fisher Distribution:
  $$X|X^\top X=C \sim D(C,KM)$$
\end{property}



